Qubit-to-Motion: Traceable Action Provenance in Hybrid QRL for Robotic Bin-Packing Sequencing

Hybrid quantum reinforcement learning has been explored for robotic decision-making, but evaluations often emphasize task success, return, or convergence, leaving unresolved whether quantum circuit outputs influence constrained actions and remain traceable through robot execution. We present \texttt{Qubit-to-Motion}, an evidence-centered framework for support-constrained sequencing and simulated robotic placement. Four Pauli-$Z$ readouts provide the sole learned input to the actor and critic, while a support mask enforces admissible object selection. Each decision is recorded and linked via step indices and SHA-256 fingerprints to a sealed route, deterministic Cartesian and inverse-kinematics waypoints, prescribed joint motion, and MuJoCo contact replay. A frozen checkpoint is evaluated across five deterministic 30-object scene variants. All 150 placements satisfy support, containment, and settling criteria. A fixed-state zero-readout intervention changes $90.0\pm0.0\%$ of decisions, demonstrating dependence on the joint circuit representation. Mean macro travel is $34.537\pm0.206$~m, inference requires $8.60\pm1.27$~ms per route, and replay achieves $8.764\pm0.220~\mu$m mean final position error with 0.356~mm maximum interpenetration. These results establish reproducible decision-to-contact traceability. The implementation is available at \href{https://anonymous.4open.science/r/Qubit-to-Motion-Quantum-Reinforcement-Learning-F7DC}{\textcolor{linkpink}{the anonymous repository}}.

==> bibliography.tex <==
\begin{thebibliography}{99}
\bibitem{wang2019stable}
F.~Wang and K.~Hauser, ``Stable bin packing of non-convex 3D objects with a robot manipulator,'' in \emph{Proc. IEEE Int. Conf. Robotics and Automation (ICRA)}, 2019, pp.~8698--8704.
\bibitem{zhao2021online}
H.~Zhao, Q.~She, C.~Zhu, Y.~Yang, and K.~Xu, ``Online 3D bin packing with constrained deep reinforcement learning,'' in \emph{Proc. AAAI Conf. Artificial Intelligence}, vol.~35, no.~1, 2021, pp.~741--749.
\bibitem{huang2022planning}
S.~Huang, Z.~Wang, J.~Zhou, and J.~Lu, ``Planning irregular object packing via hierarchical reinforcement learning,'' arXiv:2211.09382, 2022.
\bibitem{chen2020vqc}
S.~Y.-C.~Chen, C.-H.~H.~Yang, J.~Qi, P.-Y.~Chen, X.~Ma, and H.-S.~Goan, ``Variational quantum circuits for deep reinforcement learning,'' \emph{IEEE Access}, vol.~8, pp.~141007--141024, 2020.
\bibitem{jerbi2021policies}
S.~Jerbi, C.~Gyurik, S.~C.~Marshall, H.~J.~Briegel, and V.~Dunjko, ``Parametrized quantum policies for reinforcement learning,'' in \emph{Advances in Neural Information Processing Systems}, vol.~34, 2021, pp.~28362--28375.
\bibitem{skolik2022quantumagents}
A.~Skolik, S.~Jerbi, and V.~Dunjko, ``Quantum agents in the Gym: A variational quantum algorithm for deep Q-learning,'' \emph{Quantum}, vol.~6, Art.~720, May 2022.
\bibitem{hohenfeld2024quantum}
H.~Hohenfeld, D.~Heimann, F.~Wiebe, and F.~Kirchner, ``Quantum deep reinforcement learning for robot navigation tasks,'' \emph{IEEE Access}, vol.~12, pp.~87217--87236, 2024.
\bibitem{zhao2022feasible}
H.~Zhao, C.~Zhu, X.~Xu, H.~Huang, and K.~Xu, ``Learning practically feasible policies for online 3D bin packing,'' \emph{Science China Information Sciences}, vol.~65, Art.~112105, 2022.
\bibitem{zhang2025masking}
T.~Zhang, Z.~Wu, Y.~Chen, Y.~Wang, B.~Liang, S.~Moura, M.~Tomizuka, M.~Ding, and W.~Zhan, ``Physics-aware robotic palletization with online masking inference,'' in \emph{Proc. IEEE Int. Conf. Robotics and Automation (ICRA)}, 2025, pp.~6139--6145.
\bibitem{todorov2012mujoco}
E.~Todorov, T.~Erez, and Y.~Tassa, ``MuJoCo: A physics engine for model-based control,'' in \emph{Proc. IEEE/RSJ Int. Conf. Intelligent Robots and Systems (IROS)}, 2012, pp.~5026--5033.
\bibitem{schulman2017ppo}
J.~Schulman, F.~Wolski, P.~Dhariwal, A.~Radford, and O.~Klimov, ``Proximal policy optimization algorithms,'' arXiv:1707.06347, 2017.
\bibitem{lockwood2021atari}
O.~Lockwood and M.~Si, ``Playing Atari with hybrid quantum-classical reinforcement learning,'' in \emph{NeurIPS 2020 Workshop on Pre-registration in Machine Learning}, PMLR, vol.~148, 2021, pp.~285--301.
\bibitem{dragan2025continuous}
T.-A.~Dr\u{a}gan, A.~K\"unzner, R.~Wille, and J.~M.~Lorenz, ``Continuous quantum reinforcement learning for robot navigation,'' in \emph{Proc. Int. Conf. Agents and Artificial Intelligence (ICAART)}, vol.~1, 2025, pp.~807--814.
\bibitem{sinha2025navq}
A.~Sinha, A.~Macaluso, and M.~Klusch, ``Nav-Q: Quantum deep reinforcement learning for collision-free navigation of self-driving cars,'' \emph{Quantum Machine Intelligence}, vol.~7, no.~1, Art.~19, 2025.
\bibitem{nigatu2025grover}
H.~Nigatu, G.~Shi, J.~Li, J.~Wang, G.~Lu, and H.~Li, ``Quantum machine learning and Grover's algorithm for quantum optimization of robotic manipulators,'' \emph{IEEE Robotics and Automation Letters}, vol.~10, no.~12, pp.~13090--13097, Dec.~2025.
\bibitem{nigatu2026qmlrobotics}
H.~Nigatu, G.~Shi, J.~Li, G.~Lu, and H.~Li, ``Quantum machine learning for robotics: A comprehensive review of algorithms, applications, and future directions,'' \emph{Journal of Intelligent Unmanned Systems}, vol.~1, no.~1, 2026.
\bibitem{preskill2018nisq}
J.~Preskill, ``Quantum computing in the NISQ era and beyond,'' \emph{Quantum}, vol.~2, Art.~79, 2018.
\bibitem{cerezo2021vqa}
M.~Cerezo, A.~Arrasmith, R.~Babbush, S.~C.~Benjamin, S.~Endo, K.~Fujii, J.~R.~McClean, K.~Mitarai, X.~Yuan, L.~Cincio, and P.~J.~Coles, ``Variational quantum algorithms,'' \emph{Nature Reviews Physics}, vol.~3, pp.~625--644, 2021.
\bibitem{beechey2023sverl}
D.~Beechey, T.~M.~S.~Smith, and {\"O}.~{\c S}im{\c s}ek, ``Explaining reinforcement learning with Shapley values,'' in \emph{Proc. Int. Conf. Machine Learning}, PMLR, vol.~202, 2023, pp.~2003--2014.
\bibitem{brindise2024diagnostics}
N.~Brindise, A.~P.~Moreno, C.~Langbort, and S.~Trimpe, ``Pointwise-in-time diagnostics for reinforcement learning during training and runtime,'' in \emph{Proc. Learning for Dynamics and Control Conf.}, PMLR, vol.~242, 2024, pp.~694--706.
\bibitem{heese2025xqml}
R.~Heese, T.~Gerlach, S.~M\"ucke, S.~M\"uller, M.~Jakobs, and N.~Piatkowski, ``Explaining quantum circuits with Shapley values: Towards explainable quantum machine learning,'' \emph{Quantum Machine Intelligence}, vol.~7, no.~1, Art.~27, 2025.
\bibitem{huang2022masking}
S.~Huang and S.~Onta\~n\'on, ``A closer look at invalid action masking in policy gradient algorithms,'' in \emph{Proc. Int. Florida Artificial Intelligence Research Society Conf.}, vol.~35, 2022, doi:~10.32473/flairs.v35i.130584.
\bibitem{henderson2018matters}
P.~Henderson, R.~Islam, P.~Bachman, J.~Pineau, D.~Precup, and D.~Meger, ``Deep reinforcement learning that matters,'' in \emph{Proc. AAAI Conf. Artificial Intelligence}, vol.~32, no.~1, 2018.
\bibitem{agarwal2021precipice}
R.~Agarwal, M.~Schwarzer, P.~S.~Castro, A.~C.~Courville, and M.~G.~Bellemare, ``Deep reinforcement learning at the edge of the statistical precipice,'' in \emph{Advances in Neural Information Processing Systems}, vol.~34, 2021, pp.~29304--29320.
\bibitem{pineau2021reproducibility}
J.~Pineau, P.~Vincent-Lamarre, K.~Sinha, V.~Larivi\`ere, A.~Beygelzimer, F.~d'Alch\'e-Buc, E.~Fox, and H.~Larochelle, ``Improving reproducibility in machine learning research: A report from the NeurIPS 2019 reproducibility program,'' \emph{Journal of Machine Learning Research}, vol.~22, no.~164, pp.~1--20, 2021.
\bibitem{lebo2013provo}
T.~Lebo, S.~Sahoo, and D.~McGuinness, Eds., ``PROV-O: The PROV ontology,'' W3C Recommendation, Apr.~2013. [Online]. Available: \url{https://www.w3.org/TR/prov-o/}
\bibitem{martello2000three}
S.~Martello, D.~Pisinger, and D.~Vigo, ``The three-dimensional bin packing problem,'' \emph{Operations Research}, vol.~48, no.~2, pp.~256--267, 2000.
\bibitem{crainic2008extreme}
T.~G.~Crainic, G.~Perboli, and R.~Tadei, ``Extreme point-based heuristics for three-dimensional bin packing,'' \emph{INFORMS Journal on Computing}, vol.~20, no.~3, pp.~368--384, 2008.
\bibitem{wang2022dense}
F.~Wang and K.~Hauser, ``Dense robotic packing of irregular and novel 3D objects,'' \emph{IEEE Transactions on Robotics}, vol.~38, no.~2, pp.~1160--1173, 2022.
\bibitem{santos2024sequence}
A.~Santos, N.~F.~Duarte, A.~Dehban, and J.~Santos-Victor, ``Learning the sequence of packing irregular objects from human demonstrations: Towards autonomous packing robots,'' in \emph{Proc. IEEE RAS/EMBS Int. Conf. Biomedical Robotics and Biomechatronics (BioRob)}, 2024, pp.~951--957.
\bibitem{schulman2016gae}
J.~Schulman, P.~Moritz, S.~Levine, M.~Jordan, and P.~Abbeel, ``High-dimensional continuous control using generalized advantage estimation,'' in \emph{Proc. Int. Conf. Learning Representations (ICLR)}, 2016.
\bibitem{nist2015sha}
National Institute of Standards and Technology, ``Secure hash standard (SHS),'' FIPS PUB 180-4, Aug.~2015, doi:~10.6028/NIST.FIPS.180-4.
\end{thebibliography}

